Endogeneous Dynamics of Intraday Liquidity

In this paper we investigate the endogenous information contained in four liquidity variables at a five minutes time scale on equity markets around the world: the traded volume, the bid-ask spread, the volatility and the volume at first limits of the orderbook. In the spirit of Granger causality, we measure the level of information by the level of accuracy of linear autoregressive models. This empirical study is carried out on a dataset of more than 300 stocks from four different markets (US, UK, Japan and Hong Kong) from a period of over five years. We discuss the obtained performances of autoregressive (AR) models on stationarized versions of the variables, focusing on explaining the observed differences between stocks. Since empirical studies are often conducted at this time scale, we believe it is of paramount importance to document endogenous dynamics in a simple framework with no addition of supplemental information. Our study can hence be used as a benchmark to identify exogenous effects. On the other hand, most optimal trading frameworks (like the celebrated Almgren and Chriss one), focus on computing an optimal trading speed at a frequency close to the one we consider. Such frameworks very often take i.i.d. assumptions on liquidity variables; this paper document the auto-correlations emerging from real data, opening the door to new developments in optimal trading.

==> endoinfo.tex <==
%\subsubsection{model selection/performance measure}

Across this paper, our definition of ``endogenous information'' follows \cite{lam94endo}. If the price formation at our time scale (5-minute) would be efficient in the sense of the Efficient Market Hypothesis, our variables would follow martingale dynamics: their own past would not give any information on their future value.  
%Note being able to predict liquidity variables enables to predict future price changes, simply because of the documented existence of links between liquidity imbalance and future price changes [REF:lehalle-Moundji]
In such a case the best way to predict the next value of the stationarized series $y(d,\tau)$ is to take its previous value.

An Auto-Regressive modeling is a way to measure the level of information contained in the past values of the variable: in the AR model
$$y(d,\tau) = \sum_{k\geq 1} A_k y(d,\tau-k) + \epsilon(d,\tau),$$
the larger $||A||^2=\sum_{k > 1} A_k^2$, the more information in the
variable's past (since $y$ is i.i.d. if and only if $||A||^2=0$.
\comment{MB: I thought of the above and I am not sure whether $\|A\|^2$ makes sense. For instance, we can have stationary AR series with $\|A\|^2 > 1 $, e.g. if we set the characteristic polynomial to $ z^p - A_1z^{p-1} -\cdots- A_p = (z - .9)^p$ then all its roots are within unit circle, and $\|A\|^2 >>1$. }

Of course the quality of the AR model plays a role in the relevance of $||A||^2$ as a measure of the endogenous information in a variable dynamics. Note we mainly used the $R^2$ to select our models.

\comment{Table TTT provides this measure of information level in our dataset, for each of our variables. Once computed, the table should be commented}

\comment{MIKOLAJ: you should probably put a table giving figures ($||A||^2$ and $R^2$ at least) about the value of this indicator}
\comment{CHARLES-ALBERT: The table \ref{t:results} already presents results for $R^2$. For $A^2$ I am not sure, see above.}

Moreover, the vectorial version of our models is exactly the Granger causality \cite{gran88caus}. It is not the first time Granger causality is studied on 5 minutes intervals. For instance \cite{dar03idca} tested it on the joined volume $\times$ volatility dynamics and found some on the US market. At authors' knowledge, it is nevertheless the first time it is tested systematically on the three geographical zones (US, UK and Japan) and on the four liquidity variables (i.e. adding bid-ask spread and volume at best limits into the regressions).
Section \ref{sec:memory_effect} documents this kind of causality.

\comment{MIKOLAJ: In principle you should implement the Granger test in your ``causality'' sub-section, let's see how easy it is and discuss it together.}

% \comment{$R^2$}
% As we aim to quantify the endogenous information within the market, we select and present models in accordance with the out-of-sample $R^2$ statistic\footnote{\emph{R squared}, also known as \emph{coefficient of determination} for the regression problem is defined as 
% $$ R^2 = \sum_{i\in I} (y_i - \hat{y}_i)^2 \left(\sum_{i\in I} (y_i - \bar{y})^2\right)^{-1}, $$
% where $y_i, \hat{y}_i$ for $i\in I$ are respectively the ground truth and corresponding predicted values of the explained variable, while $\bar{y}$ denotes the sample mean. $R^2$ can be interpreted as the share of variance explained by the model. Note that $R^2$ is vulnerable to data preprocessing (e.g. taking logarithms of the original values); all of the results reported in this paper refer to $R^2$ in the original data space.}. 

% @article{lam94endo,
%   title={Endogenous trading volume and momentum in stock-return volatility},
%   author={Lamoureux, Christopher G and Lastrapes, William D},
%   journal={Journal of Business \& Economic Statistics},
%   volume={12},
%   number={2},
%   pages={253--260},
%   year={1994},
%   publisher={Taylor \& Francis Group}
% }
% http://people.terry.uga.edu/last/papers/jbes_1994.pdf

% @article{gran88caus,
%   title={Some recent development in a concept of causality},
%   author={Granger, Clive WJ},
%   journal={Journal of econometrics},
%   volume={39},
%   number={1},
%   pages={199--211},
%   year={1988},
%   publisher={Elsevier}
% }

% @article{dar03idca,
%   title={Intraday trading volume and return volatility of the DJIA stocks: A note},
%   author={Darrat, Ali F and Rahman, Shafiqur and Zhong, Maosen},
%   journal={Journal of Banking \& Finance},
%   volume={27},
%   number={10},
%   pages={2035--2043},
%   year={2003},
%   publisher={Elsevier}
% }
% http://xa.yimg.com/kq/groups/21741988/9865996/name/ssrn-id348820.pdf

% @article{cha00imb,
%   title={Trade size, order imbalance, and the volatility--volume relation},
%   author={Chan, Kalok and Fong, Wai-Ming},
%   journal={Journal of Financial Economics},
%   volume={57},
%   number={2},
%   pages={247--273},
%   year={2000},
%   publisher={Elsevier}
% }
% https://www.researchgate.net/profile/Wai_Ming_Fong/publication/222673190_Trade_Size_Order_Imbalance_and_the_Volatility-Volume_Relation/links/004635343514f58ba2000000.pdf

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "publication"
%%% End: 

